Learning to Act Safely with Limited Exposure and Almost Sure Certainty

This paper puts forward the concept that learning to take safe actions in unknown environments, even with probability one guarantees, can be achieved without the need for an unbounded number of exploratory trials. This is indeed possible, provided that one is willing to navigate trade-offs between optimality, level of exposure to unsafe events, and the maximum detection time of unsafe actions. We illustrate this concept in two complementary settings. We first focus on the canonical multi-armed bandit problem and study the intrinsic trade-offs of learning safety in the presence of uncertainty. Under mild assumptions on sufficient exploration, we provide an algorithm that provably detects all unsafe machines in an (expected) finite number of rounds. The analysis also unveils a trade-off between the number of rounds needed to secure the environment and the probability of discarding safe machines. We then consider the problem of finding optimal policies for a Markov Decision Process (MDP) with almost sure constraints. We show that the action-value function satisfies a barrier-based decomposition which allows for the identification of feasible policies independently of the reward process. Using this decomposition, we develop a Barrier-learning algorithm, that identifies such unsafe state-action pairs in a finite expected number of steps. Our analysis further highlights a trade-off between the time lag for the underlying MDP necessary to detect unsafe actions, and the level of exposure to unsafe events. Simulations corroborate our theoretical findings, further illustrating the aforementioned trade-offs, and suggesting that safety constraints can speed up the learning process.

==> assured_RL.tex <==
%\subsection{Barrier learning algorithm }\label{sec:assured-rl}
\juan{we do not need a change of section or subsection here}

As introduced in \eqref{eq:b_pi_opt}, our goal is to learn a safe policy $\pi$ that Barrier function $B^*(s,a)$ and therefore finds the trajectories that satisfy the constraints at all time steps almost surely. 
For this purpose we first devise an iterative algorithm that attempts to reach a fixed point satisfying \eqref{eq:bellman_for_barrier}, that would be

\begin{align}
B_{k+1}(s,a)&=\mathbb E\left[\log\left(1-D_{t+1}\right)|S_{t}=s,A_t=a\right]\\
      &+ \max_{a'\in \mathcal A} \mathbb  E\left[ B_k(s',a') |S_t=s,A_t=a\right].\label{eq:ensemble_iteration_bk}
\end{align}

Next, we appeal to the stochastic approximation machinery \cite{robbins_monro} to drop the unknown expectations yielding a data driven version \eqref{eq:ensemble_iteration_bk}. The resulting stochastic update is given in Algorithm \ref{alg:barrier}.
%This safety condition on the policy can be described by the probability $q_D^\pi(s,a)$ being null for all $s$ in the set of starting points $\mathcal S_0$, or equivalently $B^\pi(s,a)=0$ for all $s \in \mathcal{S}_0,\ a\in \mathcal A$. As before, we assume that  each state transition yields a reward $R_{t+1}$ and a damage index $D_{t+1}$, which are distributed according to the transition probability $p(s'd,r|s,a)$. {Algorithm \ref{alg:barrier} specifies how to use this data in order to learn the set of safe policies. The Barrier  function $B(s,a)$ is updated incorporating the new information about safety provided by the damage index $D_{t+1}$ at each transition}.


\begin{algorithm}[htbp]
\SetAlgoLined
% \KwData{$B$-function (iinitialized as all-zeroes)}
\KwIn{$B$-function and $(s_t,a_t,s_{t+1},d_{t+1})$ tuple}
\KwOut{Barrier-function $B$}
\vspace{-.5cm}
$$B(s_t,a_t)\leftarrow B(s_t,a_t)
+\log(1-d_{t+1})+\max_{a'}B(s_{t+1},a')$$
\KwRet{$B$}
\caption{Barrier Update}
\label{alg:barrier}
\end{algorithm}

The update in Algorithm \ref{alg:barrier} incorporates the information carried in the indicator $d_{t+1}$, about whether the constraint has been violated or not during the transition from time $t$ to time $t+1$. However, it does not only  consider  the possibility of immediate damage, but also the future effect of the action $a_t$ that is summarized in the second term  $\max_{a'}B(s_{t+1},a')$. By  repeating this update with new data coming from successive system interactions, an agent can synthesize the whole information about all past constraint violations  in the barrier function $B(s,a)$ for unveiling the set of unsafe policies.

The details of this iterative algorithm, and its performance guarantees are presented next.


% We are waiting for you in the zoom :). E.M.


\juan{the next paragraphs, including the assured algorithm and everything until "Sample complexity of Barrier learner", goes into the numericals we said }
\todo[inline]{Hancheng: Feel free to merge what I have wrote in Section ``Sample complexity of Barrier learner", but I guess that subsection title is unnecessary.}
\textcolor{red}{Then, Algorithm \ref{alg:assured_ql} uses the decomposition of Theorem \ref{thm:decomposition} to embed this safety information in the q-function $Q(s,a)$.  Hence, we identify that the condition  $Q(s,a)=-\infty$ is equivalent to $B(s,a)=-\infty$ and this propagates information about safety from successor states. Indeed,  $Q(s,a)=-\infty$ flags the pair $(s,a)$ as one leading, with nonzero probability, to imminent damage or to a next state where all further actions lead to damage. Such a pair $(s,a)$ does not comply with our requirement  of satisfying the constraints almost surely along the trajectory, and thus it is discarded from the  set of state-action pairs that ensure feasibility. This is obtained by defining safe sets $\mathcal{B}(s)$ which specify the permitted actions at state $s$. If an action is deemed \emph{unsafe} (by inspecting $Q(s,a)=-\infty$) then it is taken out from $\mathcal{B}(s)$. In this sense, at every time step we are enforcing that the set $\mathcal{B}(s)=\text{argmax}_{a} B(s,a)$.
}%red




\textcolor{red}{
This in turn  narrows the set of feasible policies that are contenders for being optimal in terms of the reward. Notice that $Q(s,a)$  also incorporates the reward, and coincides with the standard q-function when the barrier is null, so that our Assured Q-Learning algorithm learns to optimize the reward  while  assuring feasibility on the fly.      
}


\juan{can we declare that it converges or that if it converges then all states are safe? Then we could say that among the state actions that remain the effect of B is zero and Q is optimal as in the standard case? Not sure about these claims.}
\enrique{Que el Barrier Algorithm converge a.s. sale the el paper de Tsitsiklis de Q-Learning y nuestros resultados de la seccion 3. Creo que la del Q tambien sale en forma similar. La gran diferencia para mi que vale la pena investigar a futuro es que para mi el Barrier Learning Alg. converge mucho mas rapido. }


\textcolor{blue}{
\begin{remark}[Avoiding unsafe states] Keeping track of the sets of safe actions $\mathcal B(s)$   in Algorithm \ref{alg:assured_ql} implies that we can identify unsafe states as those with $\mathcal B(s)=\emptyset$. This gives us a second level of safety during training, as we  prematurely stop an episode if we reach one of  such unsafe states. In this way, we prevent what we already identified as unavoidable future damage, and assume $d=1$ for updating $B(s,a)$ and $Q(s,a)$ without actually following the trajectory until the actual damage occurs. Notice that this propagates backwards,  so that we can identify unsafe states many steps ahead of where actual damage would occur.% To illustrate this point, consider a grid walk including a tunnel with a wall at the other end, and no stopping  or backing-up actions allowed. The first time Algorithm \ref{alg:assured_ql}  explores the tunnel   and crashes to the other end,  it declares the last state unsafe, avoiding it henceforth.  Eventually, Algorithm \ref{alg:assured_ql} identifies all states in the tunnel as unsafe, avoiding entering to it at all.
\end{remark}
}


==> bckp/barrier_learning_backup.tex <==
 \subsection{Barrier learning}

Next we  focus on the feasibility problem, adding some conditions on the transition probabilities that are needed in order to derive the Barrier learner algorithm that detects unsafe policies.    Let us start by    marginalizing the transition probabilities over $R_{t+1}$ to obtain 
 $p(s',d \mid s,a) :=P(S_{t+1}=s',D_{t+1}=d \mid S_t=s,A_t=a)$.


\juan{SHOULD WE REMOVE ALL THIS RED. \\
BECAUSE ONCE WE HAVE DEFINED $D_{t+1}$ FROM THE OUTSET, THIS DOESN'T SEEM TO ADD MUCH  ANYMORE
NOT NEEDED}
\textcolor{red}{In this direction, and given the triplet $(S_t,A_t,S_{t+1})$, consider the auxiliary random variable $D_{t+1}\in\{0,1\}$ which indicates if $(S_t,A_t,S_{t+1})\in\mathcal F$, that is, $D_{t+1}=1$  if  $(S_t,A_t,S_{t+1})\in\mathcal F$ and zero otherwise. Intuitively, $D_{t+1}$ indicates if there is \emph{damage} in the transition from $S_t$ to $S_{t+1}$, and it is related to the indicator function \eqref{eq:barrier_indicator} through $D_{t+1}=\exp\left(-\mathbb I_{\left\{(S_t,A_t,S_{t+1}\in \mathcal F)\right\}}\right)$.}%blue

\textcolor{red}{Accordingly, the conditional transition probability model is augmented to incorporate this new variable, so that $p(s',d|s, a)$ represents the probability of  evolving from state $s$ to state $s'$ facing damage $d$, under action $a$. }

\juan{THIS PARAGRAPH MAY BE STILL USEFUL}
\textcolor{red}{We further make the following assumptions on  $p(s',d|s, a)$ that will allow us to learn in episodes. Specifically,  we  assume that the trajectory ends when there is damage, which is modeled by moving to an absorbent terminal state $s_D$. This state is reached the first time there is damage $D_{t+1}=1$, yielding  $D_t=0$ thereafter. Specifically, we set the following conditions on the transition probabilities
\begin{align}
&P(S_{t+1}=s_D,D_{t+1}=0| S_t \neq s_D,A_t=a_t)=0\label{eq:cond_1}\\
&P(S_{t+1}\neq s_D,D_{t+1}=1| S_t \neq s_D,A_t=a_t)=0\label{eq:cond_2}\\
&p(S_{t+1}=s_D,D_{t+1}=0| S_t = s_D,A_t=a_t)=1\label{eq:cond_3}
\end{align}
The first and second conditions state that the transition to the terminal state $s_D$ happens if and only if there is damage $D_{t+1}=1$, while the  third  condition ensures that $s_D$ is absorbent with $D_{t+1}=0$ thereafter. }%red

\textcolor{red}{Under these assumptions, we consider  the probability of violating the constraints at some point through an entire trajectory starting from $S_0=s$, with initial action $A_0=a$ and selecting subsequent actions according to a particular policy $\pi$.
\begin{align}
    q^\pi_D(s,a)&:=P\left(\bigcup_{t\geq 0} D_{t+1}=1 \Big|S_0=s,A_0=a\right)\\&=P\left(\bigcup_{t\geq 0}\{ D_{t+1}=1\}\Big| S_0=s,A_0=a\right) \label{eq:pede}
    \end{align}
We also define the expected cumulative damage starting from $S_0=s,\ A_0=a$ and following policy $\pi$ as
\begin{align}\label{eq:depi}
d^\pi(s):=    \mathbb{E}_\pi\left[\sum_{t=0}^\infty D_{t+1}=1|S_0=s,A_0=a\right]
\end{align}
It can be shown that \eqref{eq:pede} and \eqref{eq:depi} coincide~\cite{2019.Paternainyfa}. Indeed, since  conditions \eqref{eq:cond_1}-\eqref{eq:cond_3} ensure that damage $D_{t+1}$ equals one at most once in the entire trajectory, the union in \eqref{eq:pede} is disjoint, and we can write 
\begin{align}
   q_D^\pi(s,a)&=\sum_{t=0}^\infty P\left(D_{t+1}=1|S_0=s,A_0=a\right)\label{eq:pd1}\\
&=\sum_{t=0}^\infty \mathbb{E}_\pi\left[D_{t+1}=1|S_0=s,A_0=a\right]=d^\pi(s,a)\label{eq:pdsum}
\\
&=E_\pi\left[\sum_{t=0}^\infty D_{t+1}=1|S_0=s,A_0=a\right]=d^\pi(s,a)\label{eq:equivalencePDdpi}
\end{align}
The next step is to link  $q_D(s,a)$ and $d^\pi(s,a)$ with the barrier function $B^\pi(s,a)$ in \eqref{eq:b_pi}.
In the next statement we consider a policy $\pi$ which  satisfies all constraints almost surely when starting from $S_0=s$ and $A_0=a$, so that  $q_D^\pi(s,a)=0$ and prove that for such a safe policy $B^\pi(s,a)=0$.  
}

\textcolor{red}{
 \begin{theorem}
 Under conditions \eqref{eq:cond_1}-\eqref{eq:cond_3} \ $q_D^\pi(s,a)=0$ iff $B^\pi(s,a)=0$.  
\begin{proof} Starting from \eqref{eq:pd1}, and with the probabilities being non negative, we can write
\begin{align*}
&q_D^\pi(s,a)=0\\ &\Longleftrightarrow\  P(D_{t+1}=1|S_0=s,A_0=a)=0,\  \forall t\geq 0\\
   &\Longleftrightarrow\  P((S_{t},A_t,S_{t+1})\in\mathcal F |S_0=s,A_0=a)=0,\ \forall t\geq 0\\
    &\Longleftrightarrow\  \mathbb{E}_\pi\left[\mathbb I_{\left\{(S_{t},A_t,S_{t+1})\in\mathcal F\right\}}|S_0=s,A_0=a\right]=0,\ \forall t\geq 0\\ &\Longleftrightarrow\  B^\pi(s,a)=0
\end{align*}
 The second equivalence follows from the definition of $D_{t+1}$, the third one from the definition of $\mathbb I_{\{\cdot\}}$ with the  limit in \eqref{eq:v_pi_lim},  and the fourth one  from linearity and $\mathbb I_{\{\cdot\}}$ being non-positive.  
\begin{align*}
    V^\pi(s) &=\lim_{\lambda\rightarrow\infty}\mathbb{E}_{\pi}\left[\sum_{t=0}^\infty\big(\gamma^t R_{t+1}-\lambda\mathds{1}_{\left\{(S_t,A_t,S_{t+1})\not\in\mathcal{F}\right\}}\big)  ~\big|~  S_0=s\right]\nonumber
\end{align*}
\end{proof}
\end{theorem}
Finally we take advantage of the identity between $d^\pi(s,a)$ and $q_D^\pi(s,a)$ to  derive a Bellman equation for the probability of being safe. 
}%red


\begin{theorem}[Bellman equation for $q_D^\pi$]
\label{thm:Bellman}
\textcolor{red}{
Under conditions  \eqref{eq:cond_1}-\eqref{eq:cond_3} the conditional probability of violating the constraints satisfies 
 $     q_D^\pi(s,a)=\mathbb{E}\left[D_{t+1}+ q_D^{\pi}(S_{t+1},A_{t+1}) |S_t=s,A_t=a\right]$.  
}
\end{theorem}
 


\juan{ I COMMENTED THE PROOF OF THE PREVIOUS THEOREM BECAUSE IT DOESN'T FIT IN ONE COLUMN AND WE ARE NOT GOING TO USE IT ANYWAY }
 
\begin{proof} We can set the first term of \eqref{eq:pdsum} apart and identify  the  conditional expectation of $D_{t+1}$ in it
\begin{align}
     q_D^\pi(s,a)&=\sum_{\tau=t}^\infty P(D_{\tau+1}=1|S_t=s,A_t=a)\\
     &=P(D_{t+1}=1|S_t=s,A_t=a)\\&+\sum_{\tau=t+1}^\infty P(D_{\tau+1}=1|S_t=s,A_t=a)\label{eq:qdepe}
\end{align}
 By setting $Z_t=(S_t,A_t)$ to reduce notation, we  write the second term in \eqref{eq:qdepe} as
 
 
 \begin{align}
    &\sum_{\tau=t+1}^\infty P(D_{\tau+1}=1|S_t=s,A_t=a)=\sum_{\tau=t+1}^\infty\sum_{s'}\sum_{a'} P\left(D_{\tau+1}=1,Z_{t+1}=(s',a')|Z_t=(s,a)\right)\nonumber\\
    &=\sum_{\tau=t+1}^\infty\sum_{s'}\sum_{a'} P(D_{\tau+1}=1|Z_{t+1}=(s',a'),Z_t=(s,a))P(Z_{t+1}=(s',a')|Z_t=(s,a))\label{eq:Zt1Zt}
   \\&=\sum_{\tau=t+1}^\infty\sum_{s'}\sum_{a'} P(D_{\tau+1}=1|Z_{t+1}=(s',a'))P(Z_{t+1}=(s',a')|Z_t=(s,a))\label{eq:Zt1}\\
     &=\sum_{s'} \sum_{a'}q_D^{\pi}(s',a') P(Z_{t+1}=(s',a')|Z_t=(s,a))=E[ q_D^{\pi}(Z_{t+1}) |Z_t=(s,a)]
 \end{align}
 
 where we used the Markov property of the transition probability for  dropping $Z_t$ in \eqref{eq:Zt1Zt}. 
\end{proof}

The Bellman recursion in Theorem \ref{thm:Bellman} lets us compute the probability of being unsafe recursively, as the expected damage after the first transition, plus the average probability of damage starting from the next state.  As we  want to know if $q^\pi_D(s,a)=0$, we can stop if there is  damage after the first transition, and otherwise  step to the next state and repeat. This is the idea behind the barrier-learning Algorithm in next section .



\begin{theorem}[Bellman equation for $B^*(s,a)$]
\label{thm:Bellman}
 Under conditions  \eqref{eq:cond_1}-\eqref{eq:cond_3} the optimal barrier function satisfies  
 \begin{align}
      B^*(s,a)&=E\left[\mathbb I[D_{t+1}]|S_{t}=s,A_t=a\right]\\
      &+ \max_{a'\in \mathcal A}  E\left[ B^*(s',a') |S_t=s,A_t=a\right].\label{eq:bellman_for_barrier}
 \end{align}   
\end{theorem}
\begin{proof}
 It follows from Proposition 4.1.1 in \cite[pp. 217]{bersekas} under the negative assumption N.
\end{proof}
Besides providing a certificate for optimality, the Bellman's equations for $B^*(s,a)$ hints us towards a stochastic iterative algorithm to optimize \eqref{eq:b_pi_opt} from data, the same way the Q-learning  algorithm is derived from the standard unconstrained value function \cite{bertsekas}. We will elaborate on this stochastic algorithm next.
\juan{Don't we have Bertsekas DP book in the bibliography yet?} 


==> figs/corridor.tex <==
\begin{tikzpicture}[scale=.8]
\draw[fill=green!30!white] (0,0) rectangle (1,1);
\draw[fill=red!30!white] (9,0) rectangle (10,1);
\draw[step=1cm,color=gray] (0,0) grid (4,1);
\draw (4.5,.5) node{$\ldots$};
\draw[step=1cm,color=gray] (5,0) grid (10,1);
\draw[line width=2pt, purple!30!black] (0,0) --++ (4,0);
\draw[line width=2pt, purple!30!black] (0,1) --++ (4,0);
\draw[line width=2pt, purple!30!black] (0,0) --++ (0,1);
\draw[line width=2pt, purple!30!black] (10,0) --++ (-5,0);
\draw[line width=2pt, purple!30!black] (10,1) --++ (-5,0);
\draw[line width=2pt, purple!30!black] (10,0) --++ (0,1);

% \draw[line width=3pt, purple!30!black] (0,0) rectangle (4,1);
% \draw[line width=3pt, white] (4,1) -- (4,0);

\node at (.5,.45) {$s_1$};
\node at (.5+1,.45) {$s_2$};
\node at (.5+2,.45) {$s_3$};
\node at (.5+3,.45) {$s_4$};
\node at (.5+8,.45) {$s_{14}$};
\node at (.5+9,.45) {$s_{15}$};
\end{tikzpicture}

